Universal Approximation Theorems for Differentiable Geometric Deep Learning

This paper addresses the growing need to process non-Euclidean data, by introducing a geometric deep learning (GDL) framework for building universal feedforward-type models compatible with differentiable manifold geometries. We show that our GDL models can approximate any continuous target function uniformly on compact sets of a controlled maximum diameter. We obtain curvature-dependent lower-bounds on this maximum diameter and upper-bounds on the depth of our approximating GDL models. Conversely, we find that there is always a continuous function between any two non-degenerate compact manifolds that any "locally-defined" GDL model cannot uniformly approximate. Our last main result identifies data-dependent conditions guaranteeing that the GDL model implementing our approximation breaks "the curse of dimensionality." We find that any "real-world" (i.e. finite) dataset always satisfies our condition and, conversely, any dataset satisfies our requirement if the target function is smooth. As applications, we confirm the universal approximation capabilities of the following GDL models: Ganea et al. (2018)'s hyperbolic feedforward networks, the architecture implementing Krishnan et al. (2015)'s deep Kalman-Filter, and deep softmax classifiers. We build universal extensions/variants of: the SPD-matrix regressor of Meyer et al. (2011), and Fletcher (2003)'s Procrustean regressor. In the Euclidean setting, our results imply a quantitative version of Kidger and Lyons (2020)'s approximation theorem and a data-dependent version of Yarotsky and Zhevnerchuk (2019)'s uncursed approximation rates.

==> Appendices/4_Future_Research.tex <==
\section*{Future research}
Beyond the tools for building universal approximators with quantifiable performance suited to specific learning tasks, our findings raise several broader questions. We briefly outline some of these questions, which are to be the subject of future investigation.  

\hfill\\
\noindent \textbf{Optimal the width to depth ratios.} 
As described in Remark~\ref{r_narrow_vs_deep}, there is a non-trivial relationship between width and depth which has been optimized for deep ReLU networks between Euclidean geometry in \cite{pmlrv75yarotsky18a}.  Our findings suggest the question \textit{what is the optimal depth-to-width ratio} both as a function of the unknown function's regularity and the local geometries of the input and output spaces. 

\hfill\\
\noindent \textbf{Quantitative Approximation for Other Topologies}
Another direction for future work is to extend the quantitative approximation results of classical feedforward networks, for functions lying in Sobolev spaces, as obtained in \cite{Yarotski,QuantitativeDeepReLUSobolev,YAROTSKYSobolev,SIEGEL2020313}, or lying in Besov spaces, as obtained in \cite{Besov,gribonval2019approximation}, to approximation results for GDNs between a broader class metric input output spaces.  A likely point of continuation would be to exploit the well-developed literature of Sobolev spaces between metric-measures spaces, as pioneered in \cite{KorevaarSchoen1993,PiotsPekkaClassic1995Pointcareinequalityweak,HajlaszsobolMMs1996}, or the theory flourishing literature of Besov spaces with such inputs and outputs, see \cite{BesovMMs2008}.  

\hfill\\
\noindent \textbf{Non-null homotopic functions.} Theorems~\ref{thrm_homotopic_necessary_condition} and~\ref{thrm_negative_motiation} and their consequence open the way to the investigation of non-null homotopic deep neural models. Nevertheless, the construction of such networks and a method for efficiently training them is an interesting future research challenge since the recent computational topology results of \cite{MR3268623,matousek2013computing} shows that a even a computation of the possible homotopy types of a Riemannian output space is a computational challenge, of at-least $P$ complexity.  


==> Sections/Applications/K_Convergence_Classiciation.tex <==
% \subsection{Universal Sets}
% When performing binary classification, we want to learn which $x \in X$ belongs to a fixed subset $K\subseteq X$.  Thus, a classifier $\hat{c}:X\rightarrow \{0,1\}$ is typically trained to approximate $K$'s \textit{indicator function} $I_K$.  In this case, the results of \cite{farago1993strong} guarantee that, given a latent Bayesian structure on $X$, $I_K$ can be approximated point-wise with high probability.  However, even if the approximation guarantees are strengthened and $\hat{c}$ (deterministically) approximates $I_K$ point-wise, the approximation of $K$  can be incorrect. 
% \begin{ex}\label{ex_difference_pointwise}
% Let $X=[-1,1]$, $K=[0,1]$, and $\{K_k\}_{k=1}^{\infty}$ be the constant sequence of subsets of $X$ given by $K_k\triangleq (0,1)$.  Then, the pointwise limit of $I_{K_k}$ equals to $I_{(0,1)}$.  Thus, the points $\{0,1\}$ are always misclassified; even asymptotically.    
% \end{ex}
% The issue emphasised by Example~\eqref{ex_difference_pointwise} is that the points $\{0,1\}\subset K$ are limits of some sequence of points in the approximating sets $K_k$; for example, of the respective sequences $\{\frac1{k}\}_{k=1}^{\infty}$ and $\{1-\frac1{k}\}_{k=1}^{\infty}$.  Thus, a correct mode of convergence for sets should rather qualify a limiting set as containing all the limits of all sub-sequences $\{x_{k_j}\}_{j=1}^{\infty}$ where $x_k\in K_{k}$ for each $k\in\nn^+$.  

% \textit{Kuratowski upper-convergence}, introduced in \cite{KuratowskiTopology}, is a mode of convergence for sets which was specifically designed to capture this type of behaviour.  Following \citep[Definition 1.1.1]{AubinFrankowskaSetValuedAnalysis}, we say that a sequence of subsets $\{K_k\}_{k=1}^{\infty}$ of $X$ \textit{Kuratowski upper-converges} to $K\subseteq X$ if $K$ is equal to the limiting set:
% \begin{equation*}
%     \underset{k\uparrow \infty}{\operatorname{K-lim-sup}} \ K_k \triangleq \left\{
% x \in X:\, \underset{k\uparrow \infty}{\operatorname{lim-inf}}\, \|x - K_k\|=0
% \right\};
% % \label{eq_Kuratowksi}
% \end{equation*}
% where $\|x-K_k\|\triangleq \inf_{z \in K_k} \|x-z\|$.
% %
% \begin{ex}[{\citep[Example 4.12 and Theorem 4.16]{dal2012introduction}}]\label{ex_Kuratowksi_winning}
% Returning to example~\eqref{ex_difference_pointwise}, $\underset{k\uparrow \infty}{\operatorname{K-lim-sup}}\, K_k = [0,1]$.  
% \end{ex}
% Comparing Examples~\ref{ex_difference_pointwise} and~\ref{ex_Kuratowksi_winning}, we see that the Kuratowski upper-convergence does in-fact capture our intuition of a limiting set.  Moreover, the Kuratowski upper-limit of $\{K_k\}_{k=1}^{\infty}$ does not misclassify the points $\{0,1\}$, as was the case with the point-wise limit of $K's$ indicator function. 

% This is because Kuratowski upper-convergence is analogous to the uniform convergence on compacts on $\rrd$ for the correct output spaces, see \cite{TopologicalCoincidenceResults1995} for details, and therefore it is much finer than the point-wise convergence topology.  

==> Sections/Applications/Shape_Space.tex <==
\subsubsection{GDNs are Universal for Kendall's Shape Space}\label{ss_Univ_Kendall_Shape_Space}
\TBD{Replace this poop with the projective shape space...much nicer and cleaner example!}

\TBD{Some blablas about shape space and why we care}.  
Our next application shows that, when the input and output spaces are shape spaces; in the sense of \cite{kendall1984shape}, then GDNs extend the geodesic regression models of \cite{fletcher2011geodesic} to a universal geometric deep learning model.  In order to review the model of \cite{fletcher2011geodesic} and show how GDNs extend it, we begin by reviewing the shape space introduced in the landmark paper of \cite{KendallOG1984,KendallLe1993AnnalsofStats}.  


Kendall's (planar) \textit{shape space} $\Sigma_2^k$ is defined in three steps as follows.  First, any set of $k$-points $\{x_j\}_{j=1}^k$ in $\rr^2$ is identified with the following element of $\cc^k$:
$$
z_x\triangleq ((x_j)_1+(x_j)_2)_{j=1}^k
,
$$ 
where $(x_j)_1$ and $(x_j)_2$ are the coordinates of $x_j\in \rrd$.  The effect of \textit{translation} is then removed by subtracting $\bar{z_x} \triangleq \frac1{k} \sum_{i=1}^k (x_i)_1 + i(x_i)_2$ from $z_x$; this defines an element of the $2k-3$-dimensional sphere $S^{2k -3}$ called a \textit{pre-shape}.  
%
The space of \textit{pre-shapes} $S^{2k-3}$ can be endowed with a Riemannian structure in which the Riemannian exponential map about any $z \in S^{2k-3}$, and its inverse, are:
\begin{equation}
	\begin{aligned}
	\operatorname{Exp}_{S^{2k-3},z}(v) & =  \cos\left(
	\|v\|
	\right)z
	+
	\frac{\|z\|\sin(\|v\|)}{\|v\|} v
	%%
	,
	\\
	%%
	\operatorname{Exp}_{S^{2k-3},z}^{-1}(v) & = 
	\arccos\left(
	\frac{z^{\top}z }{
		\|z\|\|\tilde{z}\|
	}
	\right).
	\end{aligned}
\label{eq_pre_shape}
\end{equation}
A planar \textit{shape} $[x]\in \Sigma_2^k$ is then defined as the equivalence class:
$$
[x]\triangleq 
\{
z \in S^{2k-3}:
\,
(\exists X \in SO(2))\, zX = x
\},
$$
\fTBD{A: Check dimension}
where $SO(2)$ is the set of \textit{"orientation-preserving isometries";} i.e., $X\in SO(2)$ if $X^{\top}X = I_2$ and $\det(X)=1$.  Thus, given any $k$-tuple $x=\{x_j\}_{j=1}^k$ its \textit{shape} is the equivalence class of all other $k$-tuples which can be obtained from it by a translation followed by an orientation-preserving isometry.  

\textit{Kendall's planar shape space} $\Sigma_2^k$ is the set of all such shapes.  We make $\Sigma_2^k$ into a metric space by equipping it with the following quotient metric; which is a mild variant of the (full) \textit{Procrustean metric} of \cite{KendallLe1993AnnalsofStats}:
$$
d_p([x_1],[x_2]) \triangleq \inf_{X \in SO(2)}
d_{S^{2k-3}}(x_1,Xx_2).
$$

In  \cite{fletcher2011geodesic} and in the dedicated chapter of \cite{DrydenMardiaKendallsShapeSpaceinR2016}, the authors introduce/describe a class of regression models designed for shape analysis.  These model, which uptake pre-shape data and prediction shapes as output, are defined by:
\begin{equation}
    S^{2k-3} \ni x  \mapsto [\text{Exp}_{S^{2k-3},y_1}\circ (A\text{Exp}_{S^{2k-3},x_1}(x) + b)] \in \Sigma_2^k
    \label{eq_Flethcers_procrustean_model}
    ,
\end{equation}
where $A$ is a $k\times k$ matrix and $b \in \rrk$.  
Thus GDNs which process pre-shapes in $S^{2p-3}$ as inputs and predicting shapes as outputs are straightforward deep neural extension of the Procrustean regression model in~\eqref{eq_Flethcers_procrustean_model}.  These GDNs are (locally) defined by:
\begin{equation}
    \hat{f}: S^{2p-3} \ni x  \mapsto [\text{Exp}_{S^{2m-3},y_1}\circ g\circ \text{Exp}_{S^{2p-3},x_1}(x)] \in \Sigma_2^m
    \label{eq_Flethcers_procrustean_model}
    ,
\end{equation}
for some $g \in \NN[2p-3,2m-3]$.  

As noted in the Procrustean literature \cite{fletcher2003statistics,fletcher2011geodesic}.
\begin{corollary}\label{cor_Proc}

\end{corollary}


==> Sections/Intro/Old_intro.tex <==

\subsection*{Quantitative vs. qualitative universal approximation}
The classical universal approximation theorem for shallow feedforward networks, progressively refined in a sequence of articles by \cite{Cybenko, Hornik, Leshno, PinkusMLP}, is a \textit{qualitative} guarantee that any continuous function between Euclidean spaces can be approximated to arbitrary precision by some shallow neural network if and only if the network has nonpolynomial activation function.  Fueled by the state of the art performance achieved by deep neural network models, as opposed to their shallow counterparts, a body of literature had subsequently emerged mirroring these results but instead for deep feedforward networks of bounded width.  These began with the guarantees obtained in \cite{disconnected, Hanin, Lu, Park} for deep ReLU networks and were recently extended to feedforward networks with general non-degenerate activation functions in \cite{kidger2019universal}. 

All these results are of a \textit{qualitative} nature since they do not describe the complexity of the involved networks, as a function of their hyper-parameters, required to achieve a specific approximation quality.  This makes selecting an appropriate network structure in practice cor comparing different networks' approximation capabilities in theory challenging.  


Following the initial work of \cite{Cybenko,Hornik}, a separate branch of research began with \cite{Barron}, and subsequently refined in a series of papers \cite{mhaskar1996neural,Petrushev1999,KulsowskiBarrow2018,SIEGEL2020313} amongst others, quantifying the number of hidden neurons required for a shallow neural network to achieve a given approximation precision.  
As with the qualitative approximation results for deep feedforward networks, quantitative results for deep ReLU networks have also recently emerged in \cite{pmlrv75yarotsky18a,QuantitativeDeepReLUSobolev} describing the depth required of a deep and narrow feedforward network with ReLU activation to achieve a given level of approximation precision.  All these results are \textit{quantitative} as they specify estimates on the complexity of the involved networks' hyper-parameters required to approximate an unknown function to a prespecified level of precision.  

Currently, a quantitative version of the general qualitative universal approximation results of \cite{kidger2019universal} for deep and narrow networks with general non-pathological activation function is an open research problem in the field.  We solve this research question as a particular instance of our general quantitative results under the simplifying assumption that the input and output spaces are Euclidean.  


% Their result provides a width estimate for the approximating network but lacks an estimate of its depth. This is one of our contribution. The main difficulty here is to quantitatively prove the universal approximation theorem, on which the construction of \cite{kidger2019universal} relies. This amounts to find a rate of convergence for the Stone--Weierstrass theorem, i.e to quantify how fast polynomials approximate continuous functions defined on a compact set of $\mathbb{R}^{m}$ and taking values in $\mathbb{R}^{n}$. This is achieved by using multivariate Bernstein polynomials and a certain Bochner-type integral. Our result shows that the depth of the approximating network depends on the inverse modulus of continuity of the function being approximated, the diameter of the compact set on which the function is defined and the error of approximation that is allowed. In the case of a nonpolynomial and not infinitely differentiable function, our estimate further depends on the inverse modulus of continuity of the activation function.




==> extras.tex <==
The next lemma guarantees that locally, on any compact subset $\kkk$ of the input space $\xxx$, the Riemannian curvature $K_{\xxx}$ can be bounded.  Moreover, the Riemannian curvature $K_{\yyy}$ on any continuous image of $\kkk$ is also bounded.  
\begin{lemma}[Boundedness of Curvature]\label{lem_finitness_guarantee}
Let $\kkk$ be a non-empty compact subset of $\xxx$, $f:\xxx\rightarrow \yyy$ be continuous, and $x \in \xxx$.  Then, 
$$
\sup_{\pi_x:x\in \kkk, \,\pi \in G_{d,2}(\xxx)} 
\left|
K_{\xxx}(\pi_x)
\right|
<\infty
\mbox{ and }
\sup_{\pi_y:y\in f(\kkk), \,\pi \in G_{d,2}(\yyy)} \left|
K_{\yyy}(\pi_y)
\right|<\infty
.
$$
\end{lemma}
\begin{proof}
From the Corollary on \citep[page 167 (there is no numbering)]{BishopGeometry} since 
$\kkk$ is a compact subset of the Riemannian manifold $\xxx$, 
there exist $K \in (0,\infty)$ for which $K_{\xxx}\leq K$.  Therefore, we have the bound 
$$
\sup_{\pi_x:x\in \kkk, \,\pi \in G_{d,2}(\xxx)}  
|K_{\xxx}(\pi_x)|\leq K<\infty.
$$  

Since $f:\xxx\rightarrow \yyy$ is continuous and since $\kkk$ is compact then \citep[Theorem 26.5]{munkres2014topology} implies that $f(\kkk)$ is a compact subset of the Riemannian manifold $\yyy$.  Therefore, the Corollary on \citep[page 167]{BishopGeometry} again implies that there exists some $\tilde{K}\in (0,\infty)$ for which $K_{\yyy}\leq \tilde{K}$.  Thus, 
$$
\sup_{\pi_y:y\in f(\kkk), \,\pi \in G_{d,2}(\yyy)} |K_{\yyy}(\pi_y)|\leq\tilde{K}<\infty
.
$$
\end{proof}
